Securing Serverless Computing: Challenges, Solutions, and Opportunities

Serverless computing is a new cloud service model that reduces both cloud providers' and consumers' costs through extremely agile development, operation, and charging mechanisms and has been widely applied since its emergence. Nevertheless, some characteristics of serverless computing, such as fragmented application boundaries, have raised new security challenges. Considerable literature work has been committed to addressing these challenges. Commercial and open-source serverless platforms implement many security measures to enhance serverless environments. This paper presents the first survey of serverless security that considers both literature work and industrial security measures. We summarize the primary security challenges, analyze corresponding solutions from the literature and industry, and identify potential research opportunities. Then, we conduct a gap analysis of the academic and industrial solutions as well as commercial and open-source serverless platforms' security capabilities, and finally, we present a complete picture of current serverless security research.

==> Serverless Security [IEEE Network] (preprint)/texts/1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\IEEEPARstart{T}{he} development of cloud computing has driven various service model innovations, including serverless computing. In this model, cloud providers are responsible for all server-related management tasks, such as resource allocation, service deployment, scaling, and monitoring, and an application is charged only for its execution time. As a result, consumers can avoid tedious management tasks, focus on the business code, and save costs by not paying for idle resources. These advantages in terms of efficiency and economy have led to the rapid development of serverless computing in recent years and have attracted extensive attention from both industry and academia.
According to a recent report, the global serverless market size is estimated to grow to \$21.1 billion by 2025 \cite{serverless_market}.

% \IEEEPARstart{S}{erverless} computing is an emerging cloud service model. It outsources server-related management tasks to cloud providers, such as resource allocation, service deployment, scaling, and monitoring. Providers only charge for the resources used during code execution. Therefore, developers can focus on business code and do not need to pay for idle services. In this manner, serverless brings enormous efficiency and economic advantages to cloud applications. It has developed rapidly in the past few years and attracted extensive attention from both industry and academia.
% According to a recent report, the global serverless market size is estimated to grow to \$21.1 billion by 2025\footnote{MarketsandMarkets, ``Serverless Architecture Market Size, Share and Global Market Forecast to 2025'', 2020: http://bit.ly/serverless\_market}.

However, as a novel service model, serverless computing also has certain distinguishing features that present some challenges, leading to security and compliance concerns. For example, its agile and lightweight virtualization technologies may lead to weak isolation, and the ephemeral nature of its computing instances could increase the difficulty of security management.
In recent years, substantial efforts have been made to address these challenges. Related studies have arisen from academic research, commercial cloud providers, and thriving open-source communities and have considerably enhanced serverless security.
Therefore, a systematic survey of current research progress is needed to provide a foundation for continuing security enhancement.
% Nevertheless, they focus discretely on specific problems and lack an overall view of current research status.


%Although serverless computing's unique advantages make it widely used, some of its characteristics also pose challenges in security and privacy.
%For example, the serverless model is distinguished by the agility of lightweight virtualization technologies, but their weakness in isolation conflicts with the requirements of multi-tenant resource sharing scenarios.
% Serverless applications' fragmented boundaries and the ephemeral nature of computing instances also raise monitoring and security management challenges.
% To address these challenges, academia conducted active research; commercial cloud providers and thriving open-source communities also presented their solutions.
% These studies have considerably promoted serverless security. Nevertheless, they focus on specific problems and thus lack an overall view of current research status. Therefore, it is necessary to conduct a systematic survey of the challenges and corresponding solutions, supplemented with in-depth analysis, to provide a foundation for continuous security enhancement.

Some previous surveys of serverless computing have been conducted \cite{jonas2019cloud, shafiei2020serverless}; however, they have three main drawbacks in revealing the current status of security research. In terms of subject matter, these surveys have extensively discussed the concepts, challenges, applications, and prospects of serverless computing but have not specifically targeted security. Regarding content, the previous surveys have briefly introduced possible risks or attacks but have not systematically analyzed existing solutions and future directions of research. In terms of materials, these surveys have focused on literature work and have not considered the measures adopted in industry (i.e., commercial or open-source platforms); however, an academic focus alone is insufficient for a review of a widely applied cloud computing model such as serverless computing.
% Currently, There have been some surveys that provided overall analysis and literature reviews about serverless and its security \cite{jonas2019cloud, shafiei2020serverless}. However, they mainly focus on the concepts and application prospects; the security discussions are also inadequate.
% Besides, none of them has a systematic review of security measures applied in the industry (i.e., commercial or open-source platforms), which is largely insufficient for serverless, a young but widely applied cloud computing model.

% to the best of our knowledge, no such investigation has been performed.

%Our main objective is to investigate security challenges in serverless computing and present a systematic analysis of current solutions to facilitate future research.
Therefore, a complete and systematic review of serverless security is urgently needed. To promote serverless computing and inspire new research, we present the first survey on serverless security whose horizon is expanded from academia alone to include industry. In this paper, we first introduce the concept and background of serverless computing (\autoref{sec:background}). Starting from the unique characteristics of this service model, we then present a classification of the main security challenges and analyze their root causes. Subsequently, we review the state-of-the-art solutions proposed in the literature and adopted by popular serverless platforms for each challenge. Based on the degree to which these problems are solved, we note potential research opportunities (\autoref{sec:isolation}--\autoref{sec:confidentiality}).
%Editor: Please note that the text output by '\autoref{sec:isolation}--\ref{sec:confidentiality}' above is 'Section III--VI'; however, for grammatical correctness, it should be 'Sections III--VI'. Unfortunately, the \autoref command does not appear to have a plural functionality. Please consider either replacing the above with '\autoref{sec:isolation}--\autoref{sec:confidentiality}' (to output 'Section III--Section VI') or avoiding the use of \autoref throughout the manuscript (e.g., 'Sections \ref{sec:isolation}--\ref{sec:confidentiality}').
Finally, we illustrate our findings in comparisons of the current academic and industrial solutions as well as commercial and open-source platforms (\autoref{sec:gap}).
%Finally, we perform a gap analysis for commercial and open-source serverless platforms' security measures to illustrate the current development of serverless security in industry (\autoref{sec:gap}).

The main contributions of this work are as follows:
\begin{itemize}
\item A systematic summary of the challenges arising in securing serverless computing is presented.
\item A brief but comprehensive review of academic and industrial solutions is provided.
\item A set of promising potential research opportunities is proposed.
\item A multiaspect gap analysis of the current research status is conducted.
\end{itemize}

% Some highlights of our result include: %\xing{todo}

% \begin{itemize}
%     \item The research interests of academia and industry are relatively consistent; a series of open-source measures could help academic works be adopted smoothly.
%     \item Open-source serverless platforms lag far behind commercial platforms in terms of security; further development and standardization are urgently needed.
%     \item The amount of research work in serverless security is relatively small; more related effort is required.
% \end{itemize}

%(called \textit{functions} in serverless scenarios)



%is a cloud computing execution model where the cloud provider dynamically manages the allocation and provisioning of servers. A serverless application runs in stateless compute containers that are event-triggered, ephemeral (may last for one invocation), and fully managed by the cloud provider.
%Currently, serverless computing is gaining popularity among industry and academics due to its elasticity and economic advantage. The market s ize is estimated to grow to \$7.72 billion by 2021 \cite{serverless_market}.
%\xing{this one is better: https://www.marketsandmarkets.com/Market-Reports/serverless-architecture-market-64917099.html}
%\xue{there is another one:  the serverless market’s growth is expected to exceed \$8 billion per year by 2021, it seems that yours is better.}

\begin{figure*}[tb]
\centering
\includegraphics[width=2\columnwidth]{figures/serverless.pdf}
%\vspace{-4.5mm}
\caption{(a) A container-based FaaS technology stack. Typically, only the top-level function code is managed by customers. (b) The architecture of a serverless application that includes FaaS and BaaS components.}
%\vspace{-5mm}
\label{fig:severless}
\end{figure*}
%Editor: In this figure, please change the following: Change 'End-User' to 'End User'.


==> Serverless Security [IEEE Network] (preprint)/texts/2_background.tex <==
\section{Background and Overview}
\label{sec:background}
%In this section,


\subsection{Serverless Computing}
%\xing{working on this}



Virtualization technology is the cornerstone of cloud services.
Based on the \textit{platform-as-a-service} (PaaS) model, the recent prosperity of lightweight virtualization (e.g., \textit{containers}) has given birth to a new model: \textit{function-as-a-service} (FaaS).
As shown in \autoref{fig:severless} (a), in this model, customers develop and deploy small code pieces called \textit{functions} in the cloud. These functions are deployed in lightweight virtualized environments such as containers and executed on platform-provided runtimes. Each function focuses on a different task, and multiple functions can be combined in an event-driven manner to realize complex business logic. Events that can activate the execution of functions are called \textit{triggers}; these include but are not limited to HTTP requests, logs, storage events, and timers.

%From the developer's perspective, t
%Traditional virtual machine technology contributed to classic \textit{infrastructure as a service} (IaaS) and \textit{platform as a service} (PaaS) models. Correspondingly,

% Thanks to lightweight virtualization, functions can be initialized at an extremely fast speed (usually in a few milliseconds). Hence, providers can instantiate functions only when needed and agilely scale them, thereby maximizing resource utilization.
% This is also beneficial to consumers.
% Since the occupied resources will be released when they are not in use, consumers only need to pay for functions' actual execution time and do not need to reserve resources for emergencies.

With lightweight virtualization, functions can be initialized extremely fast (usually within a few milliseconds). Therefore, providers can instantiate functions only when needed and flexibly scale them, thereby maximizing resource utilization. Consequently, functions usually have a short lifecycle.
This agility is also beneficial to consumers.
Since the occupied resources will be released when they are not in use, consumers need to pay only for functions' actual execution time and do not need to reserve resources for emergencies.

Moreover, cloud providers offer dedicated services and application programming interfaces (APIs) for tasks such as storage, logging, and identity management. These services can help customers build and manage server-side logic, thus significantly accelerating application development and release. This service model is known as \textit{backend-as-a-service} (BaaS).

\textit{Serverless computing} is generally regarded as a combination of FaaS and BaaS. By undertaking all management tasks directly related to infrastructure resources, cloud providers make server-related details transparent to consumers. From the customer's perspective, cloud applications are serverless --- neither development, deployment, management, nor billing is server-centric. \autoref{fig:severless} (b) illustrates the architecture of a typical serverless application.



%特点



% Functions deployed in lightweight virtualized environments such as containers can be initialized within a few milliseconds.

% Through these service models, cloud providers can undertake all management tasks directly related to infrastructure resources, and make server-related detailed information transparent to consumers. This enables them to play the unique advantages of lightweight virtualization technologies truly.
% Functions deployed in lightweight virtualized environments such as containers can be initialized within a few milliseconds.
% Since they are executed in an event-driven manner, providers can instantiate functions only when needed and agilely scale them, thereby maximizing resource utilization.
% This is also beneficial to consumers.
% Since the occupied resources will be released when they are not in use, consumers only need to pay for functions' actual execution time, and do not need to reserve resources for emergencies.

%All management tasks of runtimes and functions are the provider's responsibility, such as patching, deployment, scaling, and monitoring. Therefore, developers can focus on application functionality and business logic.

% Consequently, the functions usually have a short lifecycle.

% \term{Function}: a code piece provided by the customer, running on the serverless platform, working in an event-driven manner, and usually having a short lifecycle.



%FaaS model is the core of serverless computing. Besides that, another critical part is called \textit{backend as a service} (BaaS).


% The usage measurement is also fine-grained (e.g., 0.1s). Coupled with transparent scaling, serverless is suitable for applications whose workload varies greatly. Compared with server-centric models, consumers do not need to reserve resources for emergencies nor pay for idle time.

% Therefore, providers can scale functions agilely for the highest resource utilization --- a function instance may only last for one invocation.

% , which has two distinctive characteristics:

% \textit{1) Extreme scalability.} Benefiting from lightweight virtualization, functions have fleeting initialization time (usually several milliseconds). %The scaling of function is managed by the provider.
% Therefore, providers can scale functions agilely for the highest resource utilization --- a function instance may only last for one invocation. %which is impressive in product environment.
% This feature also requires functions to be implemented as stateless. %So as to achieve the effect of scale from zero to infinity.

% \textit{2) Billing based on actual usage.}

%\textit{3) Statelessness.}



%现状

Currently, serverless computing is widely applied. Major providers such as Amazon Web Services (AWS), Microsoft Azure, and Google Cloud have all launched serverless products; a series of open-source platforms is also emerging. Meanwhile, this new cloud service model has begun to be embraced in many scenarios, such as data processing and the Internet of Things (IoT) paradigm. % , and a series of open-source platforms are emerging. %We will analyze them in detail in Section \ref{sec:platforms}.

% \oldparagraph{Terms.} For consistency and facilitating understanding, we list some terms used in this paper as follows:
% \vspace{0.02in}

% \term{Provider}: i.e., cloud provider, the provider of FaaS platforms and BaaS services.

% \term{Customer}: the user of serverless platforms and services, as well as the owner of serverless applications.

% \term{Function}: a code piece provided by the customer, running on the serverless platform, working in an event-driven manner, and usually having a short lifecycle.

% \term{Trigger}: an event that can trigger the execution of functions, including but not limited to HTTP requests, logs, storage, and timers.





% \begin{sidewaystable}

% % \begin{table*}[tb]
%     %\vspace{-1mm}
%     \caption{Security challenges, the corresponding solutions proposed in the literature and adopted in serverless platforms, and our review of their resolution status.}

%     \centering
%     \footnotesize
%     %\vspace{-1mm}
%     \scalebox{1}{
%     \begin{tabular}{l p{3.5cm} p{5cm} p{5cm} p{2cm} p{3.5cm}}
%         \toprule[1pt]
%         \makecell[c]{\textbf{Security Challenges}}&
%         \makecell[c]{\textbf{Root Cause}}& \makecell[c]{\textbf{Literature Work}} &
%         \makecell[c]{\textbf{industrial solutions}} &
%         \makecell[c]{\textbf{Status}} &
%         \makecell[c]{\textbf{Research Opportunities}}\\
%         \hline
%         \multirow{3}{*}{Resource Isolation}
%         & The usage of lightweight virtualization technologies that are weak in isolation
%         & \multirow{3}{*}{\makecell[l]{Virtual Machine-Based Secure Containers \\  - E.g., minimized VMM \cite{agache2020firecracker}, unikernel \cite{cadden2020seuss} }  }
%         & \multirow{3}{*}{\makecell[l]{Secure Containers and Network Boundary \\ - E.g., Firecracker \cite{agache2020firecracker}, gVisor, VPC}}
%         & \multirow{3}{*}{\makecell[c]{Well Resolved}} & Secure containers with better isolation, better performance, and lower overhead \\
%         \hline

%         \multirow{3}{*}{Security Monitoring}
%         & The ephemerality of functions and the broken boundaries of serverless applications
%         & \multirow{3}{*}{\makecell[l]{Information Flow Mining and Tracking \\ - E.g., static analysis \cite{obetz2019static}, dynamic \\tracking \cite{lin2018tracking,datta2020valve} }}
%         & \multirow{3}{*}{\makecell[l]{Security Scanning and Monitoring Tools \\- E.g., Azure Monitor, AWS X-Ray, \\ DevSecOps tools}}
%         &\multirow{3}{*}{Partially Resolved} & Non-intrusive tracking schemes, advanced insight capabilities like diagnosis and forensics.\\
%         \hline

%         \multirow{2}{*}{Security Management}   &    & Secure Container Network & Fine-Grained Authentication and Authorization & \multirow{2}{*}{Partially Resolved} & \\
%         & & - E.g., security enforcement network stack \cite{nam2020bastion}
%         &- E.g., IAM systems, role-based access control & & \\
%         \hline

%         % \multirow{2}{*}{C3: Third Party Functions}   & R3: Information Flow Control               & P3: Security in the Development Phase\\
%         % & \hspace{4mm} E.g., request proxy and label propagation \cite{datta2020valve,alpernas2018secure} & \hspace{3.8mm} E.g., vulnerability scanning, penetration testing...\\
%         % \hline

%         \multirow{2}{*}{Data Protection}  &  & Hardware-Based Trusted Execution Environment & Encryption in Transit and at Rest &\multirow{2}{*}{Partially Resolved} & \\
%         & &  - E.g., protecting running code with Intel SGX \cite{qiang2018se,brenner2019trust}
%         & - E.g., TLS/SSL, code/data encryption, Key Vault & & \\
%         \bottomrule[1pt]
%     \end{tabular}
%     }
%     %\vspace{-4mm}
%     \label{tab:solution}
% % \end{table*}

% \end{sidewaystable}


% \begin{sidewaystable}

\begin{table*}[tb]
\caption{The landscape of the survey, including security challenges and their root causes, proposed solutions, our reviews, and research opportunities.}
\label{tab:solution}
\footnotesize
\centering
\scalebox{0.993}{

% \begin{tabular}{l p{3.6cm} p{3.6cm} p{3.6cm} p{3.6cm}}
\begin{tabularx}{\linewidth}{lXXXX}%
\toprule[1pt]
{\makecell[c]{\textbf{Challenges}}} &
  \makecell[c]{\textbf{Resource Isolation}} &
  \makecell[c]{\textbf{Security Monitoring}} &
  \makecell[c]{\textbf{Security Management}} &
  \makecell[c]{\textbf{Data Protection}} \\ \hline
  
\rule{0pt}{8pt}\multirow{3}{*}{\makecell[l]{\textbf{Root} \textbf{Causes}}} &
  {The weakness of lightweight virtualization technologies in isolation} &
  {The ephemerality of functions and the broken boundaries of serverless applications} &
  The distributed nature of functions and the fragmented application boundaries &
  Platforms' control of the function lifecycle and BaaS services' participation in business logic \\ \hline
   
\rule{0pt}{8pt}\multirow{4}{*}{\makecell[l]{\textbf{Literature}\\\textbf{Work}}} &
  {Virtual-machine-based secure containers, e.g., minimized VMMs \cite{agache2020firecracker} and unikernels \cite{cadden2020seuss} } &
  {Information flow mining and tracing, e.g., static analysis \cite{obetz2019static} and dynamic tracing \cite{lin2018tracking,datta2020valve} } &
  {Advanced management capabilities, e.g., workflow-sensitive authorization \cite{sankaran2020workflow} and secure container network stacks \cite{nam2020bastion}} &
  {Hardware-based trusted execution environments, e.g., protecting running code with Intel SGX \cite{qiang2018se,brenner2019trust} }\\ \hline
  
\rule{0pt}{8pt}\multirow{4}{*}{\makecell[l]{\textbf{Industrial} \\ \textbf{Solutions}}} &
  {Secure containers and network boundaries, e.g., Firecracker \cite{agache2020firecracker}, gVisor, and VPCs} &
  {Security scanning and monitoring tools, e.g., Azure Monitor, AWS X-Ray, and DevSecOps tools} &
  {Fine-grained authentication and authorization, e.g., IAM systems and role-based access control} &
  {Encryption in transit and at rest, e.g., TLS/SSL, code/data encryption, and key management services} \\ \hline
  
  \rule{0pt}{8pt}\multirow{1}{*}{\makecell[l]{\textbf{Status}}} &
  {\makecell[l]{Well resolved}} &
  {\makecell[l]{Partially resolved}} &
  {\makecell[l]{Partially resolved}} &
  {\makecell[l]{Partially resolved}} \\ \hline
  
\rule{0pt}{8pt}\multirow{3}{*}{\makecell[l]{\textbf{Research}\\ \textbf{Opportunities}}} &
  Secure containers with better isolation, better performance, and lower overhead &
  Nonintrusive tracing schemes and advanced insight capabilities such as diagnosis and forensics & 
  Automatic security configuration and auditing tools & 
  Other confidential computing solutions such as homomorphic encryption \\
  \bottomrule[1pt]
\end{tabularx}
}
\end{table*}

% \end{sidewaystable}


\subsection{Threats and Security Challenges}
\label{sec:threat}



\begin{figure}[tb]
\centering
\includegraphics[width=1\columnwidth]{figures/threat.pdf}
%\vspace{-4.5mm}
\caption{Locations of threats and security challenges in the serverless computing framework. }
%\vspace{-5mm}
\label{fig:challenges}
\end{figure}

As a multitenant cloud service model, serverless computing is susceptible to security threats that can be divided into five categories based on where they are launched.
The first category consists of external attacks on applications from malicious users (\ding{172}), such as cross-site scripting attacks and injection attacks. Due to the unlimited scalability and the pay-as-you-go feature of serverless computing, denial of service attacks will lead to a substantial increase in the cost to application owners. The second comprises internal attacks on applications from malicious insiders (\ding{173}), such as illegal internal access and sniffing attacks. Adversaries in the internal network can even perceive sensitive information from the communication pattern and activity level of functions. For example, in a health monitoring application, a particular sequence of triggered functions may reflect a specific health condition of the patient \cite{shafiei2020serverless}. The remaining three categories are horizontal attacks between tenants (\ding{174}, e.g., side-channel attacks), vertical attacks on serverless infrastructures from malicious tenants (\ding{175}, e.g., container escape attacks), and vertical attacks on applications from malicious platforms (\ding{176}).


%Malicious users' external attacks on serverless applications (\ding{172}), malicious insiders' internal attacks on applications (\ding{173}), horizontal attacks between tenants (\ding{174}), malicious applications' vertical attacks on serverless infrastructures (\ding{175}), and malicious serverless platforms' attacks on applications (\ding{176}). The red arrows in \autoref{fig:challenges} depict the location of each threat in the serverless framework.

%New attacks specific to serverless computing also fall into these categories. For example, employing functions' stateless nature, adversaries may send numerous fraudulent requests to launch a resource exhaustion attack. This attack aims to increase the cost of victims (i.e., application owners) and can be classified as an external attack initiated by malicious end-users. Furthermore, adversaries in the network may also perceive sensitive information from the communication pattern and active level of functions, which can be regarded as an insider attack. For example, in a health monitoring application, a particular sequence of triggered functions may reflect a specific health condition of the patient \cite{shafiei2020serverless}.

% For example, employing functions' stateless nature, adversaries may send numerous fraudulent requests to launch resource exhaustion attacks.
% Adversaries in the network may also perceive sensitive information from the communication pattern and active level of functions. Case in point: in a health monitoring application, a particular sequence of triggered functions may reflect a certain health condition of the patient \cite{shafiei2020serverless}.

To address these threats, the best practice is to build a defense-in-depth system to protect serverless applications and platforms at multiple stages and levels. However, the flexibility and agility of serverless applications expose them to a series of security challenges in the process of achieving this goal. These challenges are concentrated in four aspects: resource isolation (\ding{182}), security monitoring (\ding{183}), security management (\ding{184}), and data protection (\ding{185}). \autoref{fig:challenges} depicts the locations of the threats and challenges in the serverless framework.

%Serverless computing reduces the cost of both providers and consumers, which seems to be a win-win situation.
% There is no such thing as a free lunch.
% The flexibility and agility of serverless computing have also brought new challenges in the security aspect, which can be summarized in four points: resource isolation, security monitoring, security management, and data protection. \autoref{fig:challenges} points out their positions in the serverless framework.


\subsection{Survey Methodology and Objects}
To fully understand the current state of the art in serverless security technologies, we collected and investigated the solutions proposed in research work and the security mechanisms adopted in practice for serverless platforms. An overview of this survey is presented in \autoref{tab:solution}.

For the literature work, we collected 77 papers related to serverless security that have been published since 2014 (when the serverless concept emerged). We selected nine recent research papers published in high-reputation conferences or journals to showcase the academic world's latest achievements.
Moreover, we collected the security features of popular serverless platforms from their documentation. These platforms include the leading commercial platforms AWS Lambda, Google Cloud Functions, Azure Functions, Alibaba Cloud Function Compute, and IBM Cloud Functions as well as the popular open-source serverless frameworks OpenFaaS, Kubeless, Knative, Fission, Apache OpenWhisk, and Nuclio.
% The supported .security features are all collected from their documentations.



% In the following sections, we first illuminate these four challenges and the corresponding solutions, respectively. Based on this analysis, we evaluate how these challenges have been resolved, and discuss potential research opportunities.
% \footnote{We only list traditional FaaS platforms. Some serverless products (e.g., Knative, Google Cloud Runs) focus on container maintenance, but do not provide function runtimes, so they are not included in our comparison. }
% \autoref{tab:platform} and \autoref{tab:opensource} display the solutions adopted by these two types of platforms, respectively.

% Note that the table only summarizes the solutions from academia and industry. The research work's actual application status will be discussed in \autoref{com:academic}.

% After that, by comparing the solutions proposed in academia and industry, as well as the techniques adopted in commercial and open-source platforms, we conduct a gap analysis and conclude this paper.

% The result is summarized in \autoref{tab:future} to motivate possible research opportunities.

% \subsection{Research Opportunities}



% Behind the prosperity, we have also heard doubts about serverless's security.
% Therefore, we extensively investigated the existing security concerns, which mainly fall in the following five categories.
%To gain an whole picture of the security situation in serverless scenarios,


% In order to fully understand the forefront of serverless security, we conducted thorough investigations in both academia and industry.
%Specifically, we collected and analyzed the solutions proposed in research works; meanwhile, we surveyed and summarized the security mechanisms used in popular serverless platforms.
% Specifically, we collected and analyzed the security solutions proposed in research works; meanwhile, we surveyed and summarized the security mechanisms adopted in popular serverless platforms.
% \autoref{tab:solution} shows these solutions and their mappings to the security concerns. % listed in Section \ref{sec:problems}.
%Next, we will elaborate on them separately.

%Then, we respectively summarize and analyze the approaches proposed by research works and the key technologies adopted in serverless platforms.





% \begin{table}[tb]
%     \caption{The status of security concerns' resolution and potential research opportunities.}
%     \centering
%     %\vspace{-1mm}
%     \scalebox{0.915}{
%     \begin{tabular}{p{3.2cm} p{1.2cm}<{\centering} p{3.9cm}}
%         \toprule[1pt]
%         \multirow{2}{*}{\textbf{Security Concerns}} & \textbf{How is} & \multirow{2}{*}{\textbf{Research Opportunities}} \\
%          & {\textbf{it solved?}} & \\
%         \hline
%         \multirow{1}{*}{C1: Resource Sharing} &  Good & O1: Better Secure Containers \\\hline
%         \multirow{1}{*}{C2: Security Management} & Fair & O2: Automated Tools\\\hline
%         \multirow{1}{*}{C3: Third Party Functions} & Good & O3: More Runtime Solutions\\\hline
%         \multirow{2}{*}{C4: Monitoring and Tracing} & \multirow{2}{*}{Fair} & O4: Non-Intrusive Solutions \\
%         && O5: Advanced Insight Capability\\\hline
%         \multirow{1}{*}{C5: Privacy and Confidentiality} & Fair & O6: More Confidential Computing\\%\hline
%         %-&-&O7: Platforms and Benchmarks\\
%         \bottomrule[1pt]
%     \end{tabular}
%     }
%     %\vspace{-4mm}
%     \label{tab:future}
% \end{table}


==> Serverless Security [IEEE Network] (preprint)/texts/4_solutions.tex <==


\oldparagraph{Countermeasures for the security concerns.} The responses to the concerns are mainly reflected in commercial platforms. 








%\paragraph{Findings and implications.}




%\xing{classify the mechanisms and map them to the research works and security concerns}

%\xue{You can adjust the format of this table later, I just want to see the effect.}




% \begin{table}[tb]
% \begin{tabular}{lllllll}
% \multicolumn{1}{c}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{Aspects}} & \multicolumn{1}{c}{\textbf{AWS Lambda}} & \multicolumn{1}{c}{\textbf{Google Cloud Functions}} & \multicolumn{1}{c}{\textbf{Azure Functions}} & \multicolumn{1}{c}{\textbf{Alibaba Function Compute}} & \multicolumn{1}{c}{\textbf{IBM Cloud Functions}} \\

% \multirow{3}{*}{Data Security} & Encryption in transit & function to filesystem, platform managent apis & support TLS & .... & support TLS & support \\
%  & Static encryption & files, secrets, environment variables & support & ... & .. & support \\
%  & isolation & Firecracker/container/microVM & ... & ... & ... & docker container \\
% \multirow{2}{*}{Operation Security} & authentication & .. & ... & ... & .. & .. \\
%  & Authorization & ... & ... & ... & .. & .. \\
% \multirow{2}{*}{Infrastructure Security} & Hardware & .. & ... & ... & .. & .. \\
%  & Software & .. & ... & ... & .. & .. \\
% \multirow{3}{*}{Monitoring} & Visualization & Amazon CloudWatch & Stackdriver Logging & Azure Monitor/application insights & CloudMonitor & sisdig \\
%  & Metrics? & .. & .. & .. & .. & .. \\
%  & Log & .. & .. & .. & .. & .. \\
% Tool & Tool &  &  & .. &  & 
% \end{tabular}
% \end{table}

==> Serverless Security [IEEE Network] (preprint)/texts/5_future.tex <==







==> Serverless Security [IEEE Network] (preprint)/texts/6_gap.tex <==
\section{Gap Analysis}
\label{sec:gap}

\renewcommand{\multirowsetup}{\centering}

\begin{table*}[tb]
    \caption{A brief list of security mechanisms used in commercial serverless platforms.}
\footnotesize
%\vspace{-1mm}
\centering
\scalebox{0.97}{
    \begin{tabular}{ll C{2.7cm}C{2.4cm}C{2.8cm}C{2.3cm}C{2.1cm}}
    % \begin{tabularx}{\linewidth}{XXXXXXX}
        \toprule[1pt]
        \multirow{2}{*}{\textbf{Aspect}} &
        \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{AWS Lambda}} & \textbf{Google} & \multirow{2}{*}{\textbf{Azure Functions}} & \textbf{Alibaba Cloud} & \textbf{IBM} \\
       & & & \textbf{Cloud Functions}& & \textbf{Function Compute} &\textbf{Cloud Functions}\\
        
        \hline
        \rule{0pt}{7.5pt}\multirow{3}{*}{\textbf{Isolation}}& \multirow{2}{*}{\textbf{System}}& \multirow{2}{*}{Firecracker} & \multirow{2}{*}{gVisor} & Azure Container Instances & Alibaba Cloud Sandbox & \multirow{2}{*}{Docker containers} \\\cline{2-7}
       \rule{0pt}{7.5pt}  & \textbf{Network} &VPC &VPC &Azure ASE &VPC &VPC  \\
        \hline
        
        \rule{0pt}{7.5pt}\multirow{2}{*}{\textbf{Monitoring}} & \multirow{1}{*}{\textbf{Visualization}} & Amazon CloudWatch & Stackdriver Logging & Azure Monitor & CloudMonitor & Sisdig \\ \cline{2-7}
        \rule{0pt}{7.5pt} & \multirow{1}{*}{\textbf{Tracing}} & AWS X-Ray & Cloud Trace & Application Insights & Context objects & Zipkin/Jaeger \\\hline
        
        \rule{0pt}{7.5pt}\multirow{5}{*}{\textbf{Management}} & \multirow{2}{*}{\textbf{Authentication}} & \multirow{2}{*}{AWS IAM} & {Cloud Functions IAM} & Azure AD and third-party identities & \multirow{2}{*}{Digital signatures} & \multirow{2}{*}{IBM IAM} \\ \cline{2-7}
        \rule{0pt}{7.5pt}& \multirow{3}{*}{\textbf{Authorization}} & Role-based/resource-based access control and other policies & \multirow{3}{2.4cm}{Role-based access control} & \multirow{3}{2.4cm}{Role-based access control} & \multirow{3}{2.4cm}{Role-based access control} & \multirow{3}{2.4cm}{Role-based access control} \\ \hline

        
        \rule{0pt}{7.5pt}\multirow{3}{*}{\textbf{Encryption}} & {\textbf{In Transit}} & mTLS & Google ALTS & mTLS & {TLS on ingress} & {TLS on ingress}\\ \cline{2-7}
        \rule{0pt}{7.5pt}& \multirow{2}{*}{\textbf{At Rest}} & Files, secrets, environment variables & \multirow{2}{*}{All data, KMS} & \multirow{2}{*}{All data, Key Vault} & Code, environment variables, KMS & \multirow{2}{*}{Data, secrets} \\  \hline
        
        
        \rule{0pt}{7.5pt}\multirow{2}{*}{\textbf{Tools}} & \multirow{2}{*}{\textbf{Tools}} & \multirow{2}{*}{AWS Trusted Advisor} & Event Threat Detection (ETD) & DevSecOps tools, Azure AD Access Reviews & \multirow{2}{*}{-} & \multirow{2}{*}{-} \\
        \bottomrule[1pt]
    \end{tabular}
    
    }
    %\vspace{-2mm}
    \label{tab:platform}
\end{table*}


\begin{table*}[tb]
    \caption{A brief list of security mechanisms used in open-source serverless platforms.}
\footnotesize
\centering
%\vspace{-1mm}
\scalebox{0.97}{
    \begin{tabular}{ll C{1.8cm}C{2cm}C{2.1cm}C{2.2cm}C{2cm}C{1.8cm}}
        \toprule[1pt]
        {\textbf{Aspect}} & {\textbf{Category}} & {\textbf{OpenFaaS}} & {\textbf{Kubeless}} & {\textbf{Knative}} & {\textbf{Fission}} & {\textbf{OpenWhisk}}  & {\textbf{Nuclio}} \\

        \hline
        
        \rule{0pt}{7.5pt}\multirow{2}{*}{\textbf{Isolation}}& \textbf{System} & Docker & Docker & Docker & {Docker} & {Docker} & Docker \\ \cline{2-8}
        \rule{0pt}{7.5pt}& \multirow{1}{*}{\textbf{Network}} & K8s namespace & K8s namespace & K8s namespace & K8s namespace & K8s namespace & K8s namespace  \\ \hline
        
        \rule{0pt}{7.5pt}\multirow{2}{*}{\textbf{Monitoring}} & {\textbf{Visualization}} & Grafana & Grafana & Grafana & Grafana & Kamon & Dashboard \\ \cline{2-8}
        \rule{0pt}{7.5pt}& {\textbf{Tracing}} & - & - & Zipkin/Jaeger & Zipkin/Jaeger & Zipkin/Jaeger & -  \\\hline
        
        \rule{0pt}{7.5pt}\multirow{3}{*}{\textbf{Management}} & \multirow{2}{*}{\textbf{Authentication}} & \multirow{2}{*}{OAuth2} & Kong authentication &  Istio authentication& \multirow{2}{*}{DID key method} & Self-hosted authentication  & \multirow{2}{*}{-} \\ \cline{2-8}
        \rule{0pt}{7.5pt}& \multirow{1}{*}{\textbf{Authorization}} & K8s RBAC & K8s RBAC & K8s/Istio RBAC & K8s/Istio RBAC & Support  & - \\ \hline
        
        \rule{0pt}{7.5pt}\multirow{2}{*}{\textbf{Encryption}} & \multirow{1}{*}{\textbf{In Transit}} & {TLS on ingress} &{TLS on ingress} & Istio mTLS & Istio mTLS &{TLS on ingress}&{TLS on ingress}\\ \cline{2-8}
        \rule{0pt}{7.5pt}& \multirow{1}{*}{\textbf{At Rest}} & K8s secrets & K8s secrets & K8s secrets & K8s secrets & K8s secrets & K8s secrets\\

        \bottomrule[1pt]
    \end{tabular}
    }
    %\vspace{-4mm}
    \label{tab:opensource}
\end{table*}

% \begin{comment}


% \begin{table*}[tb]
%     \caption{A comparison of security mechanisms used in commercial and open-source serverless platforms.}
% \footnotesize
% %\vspace{-1mm}
% \centering
% \scalebox{1}{
%     \begin{tabular}{l p{7.9cm} p{7.3cm}}
%         \toprule[1pt]
%         \makecell[c]{\textbf{Aspect}} & \makecell[c]{\textbf{Commercial Platforms}} & \makecell[c]{\textbf{Open-Source Platforms}}\\
%         \hline

%         \multirow{2}{*}{\textbf{Isolation}}
%         & {Provide secure containers for isolation (e.g., Firecracker \cite{agache2020firecracker}, gVisor); use VPC for network-level isolation}
%         & {Use Docker container for isolation and Kubernetes namespace as network boundary}\\\hline

%         \multirow{3}{*}{\textbf{Monitoring}}
%         & {Provide specialized monitoring and tracking tools (e.g., AWS X-Ray, Google Cloud Trace); can be connected to consoles for visualization (e.g., Amazon CloudWatch, Google Stackdriver, Azure Monitor)}
%         & \smallskip\vspace{-2mm}{Compatible with open-source tracking tools (e.g., Zipkin, Jaeger) and open source visualization tools (e.g., Grafana)}\\\hline

%         \multirow{3}{*}{\textbf{Management}}
%         & {Provide IAM systems, but can also be connected to third-party authentication systems; have own access control policies (mostly role-based), and some platforms provide multiple kinds of polices}
%         & {Support third-party identity management system (e.g., Kong Authentication); employ the authorization mechanism provided by the infrastructures (i.e., Kubernetes/Istio RBAC)}\\\hline

%         \multirow{2}{*}{\textbf{Encryption}}
%         & {Support encryption for inter-function communications and customer-uploaded code/files; provide KMS tools for secret management}
%         & {Support TLS via ingress gateways, utilize Kubernetes Secrets to manage sensitive information}\\\hline

%         \multirow{2}{*}{\textbf{Tools}}
%         & {Provide various security tools (e.g., AWS Trust Advisor, Google Event Threat Detection, Azure AD Access Reviews)}
%         & \multirow{2}{*}{Can be integrated with third-party tools}\\

%         \bottomrule[1pt]
%     \end{tabular}
%     }
%     %\vspace{-2mm}
%     \label{tab:platform}
% \end{table*}
% \end{comment}

During our investigation, we obtained some interesting findings about the current research status of serverless security, which may imply potential directions towards a better ecosystem.
%In this section, we perform comparisons between academic and industrial solutions, as well as the security measures in commercial and open-source platforms, to illustrate our main findings.

\subsection{Academic Solutions vs. Industrial Solutions}
\label{com:academic}
We compared the efforts in academia and industry from three perspectives: research interests, features of the solutions, and application status.
As mentioned above, both academic and industrial solutions cover the four main security challenges. This consistency in research interests implies that the current research is in a healthy state.

Nonetheless, the solutions show different characteristics. Academic research tends to demonstrate the feasibility of using specific methods, especially new technologies, to solve particular problems.
In contrast, the goal of commercial platforms is to be as secure as possible while ensuring stability. Thus, providers prefer methods that have been proven in long-term practice and usually combine several methods to achieve multilayer protection. In addition, research-led solutions often adopt a more holistic approach, from developer to platform. Without control over other parties, providers can promote their solutions only through guidelines or best practices.

Regarding application status, some of the reported academic research work has not yet been tested or applied in industry, as it is relatively new. We believe that open-source efforts from both academia and industry, such as publicly available research, real-world datasets, and standardized benchmarks, can help promote smooth adoption of newly emerging solutions.

% % Note that we regard Firecracker \cite{agache2020firecracker} as an industrial work since it entirely comes from AWS.

% \autoref{test}
%    \item Current serverless security research is healthy; a series of open-source measures could help academic works be adopted smoothly.
%    \item Open-source serverless platforms lag far behind commercial platforms in terms of security; further development and standardization are urgently needed.
%    \item The amount of work in serverless security is relatively small; more related work is required.

%\paragraph{Finding 1: Current serverless security research is healthy.}
% \begin{comment}

% We compared academia and industry's efforts on serverless security from three aspects: research interests, features of the solutions, and application status.
% As aforementioned, both academic and industrial solutions cover the four main security challenges of serverless computing. This consistency in research interests implies that the current research is in a healthy state.

% Nonetheless, their key focuses are quite different. Academic research tends to demonstrate the feasibility of using specific methods, especially new technologies, to solve particular problems.
% However, the goal of commercial platforms is to be as secure as possible while ensuring stability. Thus providers prefer methods that have been proven in long-term practice, and usually combine several methods to achieve multi-layer protection. Besides, the research-led solutions are often a more holistic approach from the developer to the platform. Without control over other parties, providers can only promote their solutions through guidelines or best practices.

% Regarding the application, some novel research work has not yet been tested and applied by the industry. Meanwhile, some research work led by industry achieved success in academia due to large-scale experimental verification. We believe that several open-source efforts could help research work get adoption smoothly:
% (1) open-source data (e.g., actual workloads) can enable academia to gain more industrial insights to conduct more practical research;
% (2) open-source benchmarks, especially large-scale benchmark applications, are conducive to more solid evaluations;
% (3) open-source research and standardized open-source platforms can help providers accelerate the adaptation of academic work. % and producing more valuable work. % and benefit academia in producing more valuable work.

% %\paragraph{Finding 2: Academic research have not been applied in practice.}
% %Since these works are relatively new, this point may require longer-term observation.
% %For example, as many studies are not open-source or only implemented on open-source platforms, providers need further adaptation and evaluation to apply academic research to practice.
% %Besides, the production environment is more complex than the experimental one, thus some assumptions may also need to be adjusted.

% \end{comment}
\subsection{Commercial Platforms vs. Open-Source Platforms}
\label{sec:platforms}

% During the investigation, we get some impressions about the current research status of serverless security, which may imply potential directions towards a better ecosystem. In this section, we perform comparisons between academic and industrial solutions, as well as the security measures in commercial and open-source platforms, to illustrate our main findings.
Various commercial and open-source serverless platforms have flourished thanks to the vigorous serverless computing market. During our investigation, we found considerable differences in security between these two kinds of platforms. We discuss and analyze this phenomenon in this section.
Specifically, we compare the security measures adopted in commercial and open-source platforms in terms of five aspects: isolation, monitoring, management, encryption, and tools. The detailed results are listed in \autoref{tab:platform} and \autoref{tab:opensource}.
% Serverless computing's vigorous development has promoted the establishment of many commercial and open-source platforms.



% Note that not all
% \begin{table*}[tb]
%     \caption{A brief list of security mechanisms used in commercial serverless platforms.}
% \footnotesize
% %\vspace{-1mm}
% \centering
% \scalebox{0.879}{
%     \begin{tabular}{C{1.6cm}C{1.9cm}C{2.8cm}C{2.9cm}C{2.8cm}C{2.8cm}C{2.8cm}}
%         \toprule[1pt]
%         \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Aspect}} & \multirow{2}{*}{\textbf{AWS Lambda}} & \textbf{Google} & \multirow{2}{*}{\textbf{Azure Functions}} & \textbf{Alibaba} & \textbf{IBM} \\
%         & & & \textbf{Cloud Functions}& & \textbf{Function Compute} &\textbf{Cloud Functions}\\

%         \hline

%         \multirow{4}{*}{\textbf{Data}} & \multirow{1}{*}{\textbf{Encryption in transit}} & Support & Support & Support & Support & Support\\ \cline{2-7}
%         \multirow{4}{*}{\textbf{Security}} & \multirow{2}{*}{\textbf{Encryption at rest}} & Files, secrets, environment variables & \multirow{2}{*}{All data, KMS} & \multirow{2}{*}{All data, Key Vault} & Code, environment variables, KMS & \multirow{2}{*}{Data, secrets} \\ \cline{2-7}
%          & \multirow{2}{*}{\textbf{Isolation}} & \multirow{2}{*}{Firecracker/VPC} & \multirow{2}{*}{gVisor/VPC} & Azure Container Instances/ASE & Alibaba cloud sandbox/VPC & \multirow{2}{*}{Docker container/VPC} \\ \hline
%         \multirow{3.5}{*}{\textbf{Operation}} & \multirow{2}{*}{\textbf{Authentication}} & \multirow{2}{*}{AWS IAM} & \multirow{2}{*}{Cloud Functions IAM} & Azure AD and third-party identities & \multirow{2}{*}{Digital signature} & \multirow{2}{*}{IBM IAM} \\ \cline{2-7}
%         \multirow{2}{*}{\textbf{Security}} & \multirow{3}{*}{\textbf{Authorization}} & Role-based/resource-based access control and other policies & \vspace{0.2mm} Role-based access control & \vspace{0.2mm} Role-based access control & \vspace{0.2mm} Role-based access control & \vspace{0.2mm} Role-based access control \\ \hline
%         \multirow{1}{*}{\textbf{Infrastructure}} & \multirow{1}{*}{\textbf{Hardware}} & Data center security & Data center security & Data center security & Data center security & Data center security \\ \cline{2-7}
%         %\multirow{2}{*}{\textbf{Security}}& \multirow{2}{*}{\textbf{Software}} & Automatic patching, but not for custom runtimes & Automatic patching, not support custom runtimes & Automatic patching, but not for custom runtimes & Automatic patching, but not for custom runtimes & Automatic patching, but not for custom runtimes \\ \hline
%         \multirow{1}{*}{\textbf{Security}}& \multirow{1}{*}{\textbf{Software}} & \multicolumn{5}{c}{Platforms provide maintenance and patching for supported runtimes, but not for custom runtimes.} \\ \hline
%         \multirow{5}{*}{\textbf{Monitoring}} & \multirow{1}{*}{\textbf{Visualization}} & Amazon CloudWatch & Stackdriver Logging & Azure Monitor & CloudMonitor & Sisdig \\ \cline{2-7}
%         & \multirow{1}{*}{\textbf{Metrics}} & \multicolumn{5}{c}{Statistics and performance metrics}  \\ \cline{2-7}
%          & \multirow{2}{*}{\textbf{Logging}} & Integration, storage, and access & Recording, viewing, and response & Query, analysis, and response & \multirow{2}{*}{Query and response} & Viewing, recording, and event tracking \\ \cline{2-7}
%          & \multirow{1}{*}{\textbf{Tracing}} & AWS X-Ray & Cloud Trace & Application Insights & Context object & Zipkin/Jaeger \\\hline
%         \multirow{2}{*}{\textbf{Others}} & \multirow{2}{*}{\textbf{Tools}} & \multirow{2}{*}{AWS Trusted Advisor} & Event Threat Detection (ETD) & DevSecOps tools, Azure AD Access Reviews & \multirow{2}{*}{-} & \multirow{2}{*}{-} \\
%         \bottomrule[1pt]
%     \end{tabular}

%     }
%     %\vspace{-2mm}
%     \label{tab:platform}
% \end{table*}


% \begin{table*}[tb]
%     \caption{A brief list of security mechanisms used in open-source serverless platforms.}
% \footnotesize
% \centering
% %\vspace{-1mm}
% \scalebox{0.915}{
%     \begin{tabular}{C{1.6cm}C{2.2cm}C{1.8cm}C{2.5cm}C{2.05cm}C{3cm}C{1.6cm}C{1.6cm}}
%         \toprule[1pt]
%         \multicolumn{1}{c}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{Aspects}} & \multicolumn{1}{c}{\textbf{OpenFaaS}} & \multicolumn{1}{c}{\textbf{Kubeless}} & \multicolumn{1}{c}{\textbf{Fission}} & \multicolumn{1}{c}{\textbf{OpenWhisk}} & \multicolumn{1}{c}{\textbf{Fn Project}} & \multicolumn{1}{c}{\textbf{Nuclio}} \\

%         \hline

%         \multirow{3}{*}{\textbf{Data}} & \multirow{1}{*}{\textbf{Encryption in transit}} & \multicolumn{6}{c}{Simply support TLS via ingress gateways}\\ \cline{2-8}
%         & \multirow{1}{*}{\textbf{Encryption at rest}} & K8s secrets & K8s secrets & K8s secrets & K8s secrets & - & K8s secrets\\ \cline{2-8}
%         \multirow{1.5}{*}{\textbf{Security}} & \multirow{2}{*}{\textbf{Isolation}} & Docker/K8s namespace & Docker/K8s namespace & Docker/K8s namespace & \multirow{2}{*}{Docker/K8s namespace} & \multirow{2}{*}{Docker} & Docker/K8s namespace \\ \hline
%         \textbf{Operation} & \multirow{1}{*}{\textbf{Authentication}} & OAuth2 & Kong Authentication & DID key method & Self-hosted authentication & - & - \\ \cline{2-8}
%         \textbf{Security} & \multirow{1}{*}{\textbf{Authorization}} & K8s RBAC & K8s RBAC & K8s/Istio RBAC & Support & - & - \\ \hline

%         \textbf{Infrastructure Security} & \multirow{2}{*}{\textbf{Software}} & \multicolumn{6}{c}{\multirow{2}{*}{Communities provide maintenance and patching for a set of supported runtimes.}} \\ \hline

%         \multirow{4}{*}{\textbf{Monitoring}} & \multirow{1}{*}{\textbf{Visualization}} & Grafana & Grafana & Grafana & Kamon & Grafana & Dashboard \\ \cline{2-8}
%         & \multirow{1}{*}{\textbf{Metrics}} & \multicolumn{6}{c}{Basic statistics and performance metrics} \\ \cline{2-8}
%          & \multirow{1}{*}{\textbf{Logging}} & Access & Access & Access & Access & Access & Access \\ \cline{2-8}
%          & \multirow{1}{*}{\textbf{Tracing}} & - & - & Zipkin/Jaeger & Zipkin/Jaeger & Zipkin/Jaeger & -  \\
%         \bottomrule[1pt]
%     \end{tabular}
%     }
%     %\vspace{-4mm}
%     \label{tab:opensource}
% \end{table*}

% To obtain security measures used in practice, we studied security mechanisms and technologies used in leading commercial serviceless platforms: AWS Lambda, Google Cloud Functions, Azure Functions, Alibaba Function Compute, and IBM Cloud Functions, and popular open-source serverless frameworks: OpenFaaS, Kubeless, Fission, Apache OpenWhisk, Fn Project, and Nuclio. \autoref{tab:platform} and \autoref{tab:opensource} display the solutions adopted by these two types of platforms, respectively.


% Note that we only list traditional FaaS platforms. Other serverless products (e.g., Google Cloud Runs) focus on container maintenance, but do not provide function runtimes, so they are not included in our comparison.


% https://aws.amazon.com/lambda/
% https://cloud.google.com/functions
% https://azure.microsoft.com/en-us/services/functions/
% https://cloud.ibm.com/functions/
% https://www.alibabacloud.com/products/function-compute

% https://www.openfaas.com/
% https://kubeless.io/
% https://knative.dev/
% https://fission.io/
% https://nuclio.io/
% https://openwhisk.apache.org/
% https://fnproject.io/

First, most commercial platforms are equipped with self-developed secure containers and provide VPCs for network-level isolation. In terms of monitoring, they introduce their own specialized distributed tracing and monitoring products into serverless scenarios and connect them to unified visualization consoles. Through security policies and IAM systems, these platforms provide mature authentication and authorization capabilities and support data encryption via storage services. Furthermore, their long-term investment and technological accumulation allow commercial platforms to provide many tools to assist customers, such as configuration recommendation and risk detection.

In contrast, most open-source platforms are built atop Kubernetes (K8s). Therefore, standard Docker containers and K8s namespace-based network isolation have become a general technical solution. For monitoring, these platforms usually integrate third-party tools or employ their infrastructures' capabilities to avoid reinventing the wheel. Moreover, open-source platforms mainly rely on ingress gateways and infrastructures such as K8s and Istio to achieve security management and encryption in transit. The secret management task is also outsourced to the underlying K8s infrastructure.
Similar to the monitoring aspect, open-source platforms usually do not provide security tools natively but support the integration of third-party tools such as Jenkins.


% Data security mechanisms include data encryption in transit and at rest, which involves key management and the encryption of user-uploaded data (e.g., function code). Isolation mechanisms (i.e., virtualization technologies) also fall into this category.
% Thanks to mature storage services and security management experience, commercial platforms provide adequate support for encryption in transit and at rest. They also provide standard key management services (KMS) to help users deal with secrets.



% With mature identity access management (IAM) systems, commercial platforms usually provide well-defined identity authentication and fine-grained authorization policies.


% Infrastructure security mechanisms describe security measures for hardware and software infrastructures. Commercial platforms are hosted from the physical layer to function runtimes. They support a set of runtimes officially and maintain the entire technology stack's update. Unlike them, open-source platforms only provide the software stack above container platforms. The communities are responsible for maintaining the supported runtimes. Neither commercial nor open-source platforms provide maintenance for custom runtimes.

% As for monitoring, we considered visualization tools, supported metrics, log operations, and tracing mechanisms. Commercial platforms provide fantastic tools to aggregate, display, and analyze monitoring data and logs. %, and regard them as an essential selling point. These tools have different implementations and capabilities.
% Some of them can even work as triggers for automatic function management.
% However, open-source platforms usually integrate with third-party tools to avoid reinventing the wheel. Fission's tracing capability also comes from the underlying Istio infrastructure.

% Other mechanisms refer to other available security tools.

In terms of the above five aspects, the security measures of commercial platforms are all stronger than those of open-source platforms in terms of completeness and richness. The latter's security capabilities mainly rely on infrastructure or third-party tools.
Two main reasons for this difference exist.
First, commercial platforms have richer cloud management experience and more capital and human resources, so they can leverage their existing security mechanisms and provide standardized features as BaaS services (e.g., IAM systems). Second, the development of open-source platforms is still relatively rudimentary. They focus more on realizing core features of serverless computing, such as agile application construction and automatic function scaling, rather than security features.
% Commercial providers have adopted many security measures with the experiences in operating cloud services and offered some standard features as BaaS services (e.g., IAM systems). This makes them far ahead of open-source platforms in security.

Mature and standardized open-source platforms can counter the vendor lock-in problem and stimulate community efforts and related work.
Nevertheless, open-source platforms still have a long way to go to compete with commercial platforms in terms of security.
This security lag also limits their application.
Hence, more effort is needed to develop and standardize the security mechanisms of open-source serverless platforms. Although some have taken the lead (e.g., OpenFaaS), the competition among open-source serverless platforms is still fierce, and there is no de facto standard. From this perspective, unremitting efforts in developing security measures and the establishment of unique security capabilities therewith may become the key to gaining the dominant position.


% Therefore, more effort is needed to further research and standardize the security mechanisms of open source serverless platforms.


% \subsection{Researches on Serverless Security vs. Research in Other Fields}


% \paragraph{Finding 3: The amount of research works in serverless security is small.}
%Although many excellent serverless security works have emerged recently, the amount of security research is still small.
% This paper basically covers all primary research on serverless security.
% This quantity is essentially insufficient, especially compared with areas that have been well studied.
% Therefore, with the booming of serverless computing, more research work is needed to advance the state of the art.

%First, popular open-source platforms are a critical countermeasure for vendor lock-in problems. However, the huge gap between them and commercial platforms in terms of security undoubtedly limits their applications. %However, as shown in Section \ref{sec:platforms}, there is a huge gap between the security measures of current open-source and commercial platforms.
%Consequently, even if providers adopt open-source platforms, there will still be ``security vendor lock-in'' issues due to their reliance on providers' security services.
%Therefore, they should actively research and integrate open-source security mechanisms to compete with commercial platforms. This is also favorable for academic researches since they are usually conducted on open-source platforms.

%In addition, the current lack of open-source serverless benchmarks, especially large-scale benchmark applications, also greatly hindered academic research. Without actual workloads and realistic evaluation cases, it is difficult for academia to produce valuable results. Therefore, any effort made in this area will certainly benefit related work.
%Academic researches are bound to benefit a lot from this type of research.


==> Serverless Security [IEEE Network] (preprint)/texts/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper has presented a survey of both literature research and industrial solutions to elucidate the research status of techniques for securing serverless computing. Starting from the characteristics of serverless environments, we explained the origins of four main security challenges: resource isolation, security monitoring, security management, and data protection. Based on a review of existing solutions, we then identified possible research directions. Finally, we compared academic and industrial solutions as well as current commercial and open-source serverless platforms and elaborated on our thoughts regarding promising directions for establishing a better research and application ecosystem.


% In this paper, we presented a survey of the challenges, solutions and opportunities for securing serverless computing. From the We first provided the background of this cloud service model and classified its major security challenges. In response to these concerns, we thoroughly analyzed the solutions proposed in research work and security measures adopted in commercial and open-source serverless platforms. Based on them, we discussed the potential research opportunities and analyzed the gap towards a healthier research ecosystem.
% We look forward to more valuable research work in this promising field.


% Despite the rising interest and expectations on serverless computing, there isn't a proportional number of research articles on its security just yet.

==> Serverless Security [IEEE Network] (preprint)/texts/challenge_1_isolation.tex <==
\section{Challenge 1: Resource Isolation}
\label{sec:isolation}
Serverless computing relies on the dynamic release and reuse of software and hardware to improve resource utilization and reduce costs. Thus, there is a strong requirement for resource isolation, especially among multiple tenants.

However, this requirement conflicts with the weak isolation of lightweight virtualization, thereby giving rise to this challenge.
Serverless computing requires swift and on-demand function initialization. To this end, lightweight virtualization technologies have been widely adopted.
Unlike traditional virtual machines (VMs) with guest operating systems (OSs), containers share the host's OS kernel, and thus, their isolation is weak.
Malicious consumers could employ this weakness to influence or attack other consumers located on the same host (e.g., via side-channel attacks). For example, Wang \textit{et al.} \cite{wang2018peeking} found that AWS Lambda suffers from performance isolation issues, and Azure Functions has placement vulnerabilities that facilitate side-channel attacks.

% \paragraph{C1: Multi-tenant resource sharing cause security risks.}
% Reuse is the key to improve resource utilization and reduce costs.
% Thus, providers actively shrink the number of function instances, even to zero, when they are inactive.
% The released resources are supplied to active workloads. Nevertheless, the multi-tenant sharing of hardware and software resources allows malicious consumers to influence or attack other consumers located on the same host (e.g., via side-channel attacks).
% Besides, lightweight virtualization technologies like containers are relatively weak in isolation, which aggravates the risk of resource sharing.
%Besides, achieving such agility while ensuring service quality requires functions can be instantiated in an extremely short time. To this end, providers tend to use lightweight virtualization approaches, such as containers. However, they are relatively weak in security and isolation, which aggravates the risk of resource sharing.

%是否要详细举例

%like Rowhammer


% \paragraph{R1: Virtual Machine Based Isolation.}
\soa To enhance the isolation of lightweight virtualization technologies and address this challenge, published research focuses on VM-based solutions. Compared with containers, VMs can provide better security boundaries but require a longer time to initialize. Hence, researchers have attempted to make VMs more lightweight to meet the flexibility requirements of serverless computing.
% To address the security concern raised by multi-tenant resource sharing, researchers proposed virtual machine based isolation.
% Different from typical containers that share the host kernel, each virtual machine has a guest kernel, which reduces the attack surface and provides a better security boundary.
% To apply virtual machines in serverless scenarios that emphasize flexibility, existing works attempt to make virtual machines more lightweight.
The basic idea is to reduce the size of the guest kernels, that is, remove unnecessary modules, to build ``microVMs'', even keeping only the libraries that will be used \cite{agache2020firecracker,cadden2020seuss}. Moreover, Cadden \textit{et al.} \cite{cadden2020seuss} employed unikernel snapshots to further accelerate initialization, and Agache \textit{et al.} \cite{agache2020firecracker} minimized virtual machine monitors (VMMs) to reduce the trusted computing base. These microVMs have successfully reduced the initialization time to the millisecond level while providing VM-level isolation.


%In order to achieve rapid deployment and high-density caching of serverless functions, Cadden et al. present SEUSS \cite{cadden2020seuss}, a system-level solution, which deploys functions from unikernel snapshots to shorten the start time of functions. Besides, SEUSS applies page-level sharing across snapshot stacks to reduce the memory footprint. Moreover, Cadden et al. fully consider the security of SEUSS. They use unikernel and restrict sharing to read-only pages to provide isolation, and reduce the number of interfaces to limit the attack surface area. However, the use of page-sharing makes the system vulnerable to memory-based side-channel attacks and hardware-level attacks.

\ins Led by Amazon, Firecracker \cite{agache2020firecracker} has been applied in AWS Lambda. Moreover, all surveyed commercial serverless platforms except IBM Functions utilize their own \textit{secure container} products. These containers enable advanced isolation by employing various techniques, such as microVMs (e.g., Firecracker) and container sandboxes (e.g., gVisor). Commercial platforms also provide mechanisms for network-layer isolation, such as \textit{virtual private clouds} (VPCs).
% Different from them, the standard docker container and Kubernetes namespace-based network isolation dominate open-source platforms.


% \paragraph{P1: Secure Container Technologies and Network Boundary.

\rev
Secure containers provide VM-level resource isolation and have become a standard mode of implementation in production environments. Therefore, we consider this challenge well resolved.
However, due to hardware sharing, these approaches are still susceptible to side-channel attacks. Moreover, trade-offs remain between security and performance. For example, gVisor sacrifices significant performance for security (in particular, a 216$\times$ reduction in file opening speed) \cite{young2019true}.
Additionally, many existing efforts employ snapshots \cite{ustiugov2021benchmarking} or even memory sharing \cite{cadden2020seuss} to reduce the start-up time as much as possible, which also degrades security to a certain extent.

\reo
Looking forward, serverless computing will embrace new secure containers if they offer progress in the following three dimensions: (1) security, achieving better isolation than VMs; (2) efficiency, providing performance closer to that of physical machines; and (3) lightweight computing, incurring lower overheads.

% In serverless scenarios, performance shortcomings can be compensated by high concurrency. Virtualization technology's agility, especially initialization time, has become a dominating factor affecting service quality. 
% Nevertheless, many studies aiming at this sacrificed security to some content 
% Hence, better secure containers with less start-up time and higher isolation are a future research opportunity. 

==> Serverless Security [IEEE Network] (preprint)/texts/challenge_2_monitoring.tex <==
\section{Challenge 2: Security Monitoring}
\label{sec:detection}

A serverless platform generally maintains a set of runtimes for functions, including commonly used packages of the supported programming languages.
Moreover, to meet diverse development needs, most providers also support custom runtimes and even provide function marketplaces.
The security risks posed by third-party packages and functions necessitate reliable monitoring capabilities to detect anomalies and determine the security status.

Furthermore, in a serverless environment, the ephemeral nature of functions and the broken application boundaries present new challenges.
First, although the short-lived nature of functions reduces the attack surface, it also significantly narrows the window for developers to discover and diagnose problems.
Second, as shown in \autoref{fig:severless} (b), a serverless application may have multiple entry points due to a variety of triggers. These entry points, coupled with BaaS services, cause the boundaries of serverless applications to be fragmented and further increase the difficulty of monitoring.
Moreover, lacking control over the execution environments and BaaS services, consumers must rely on the provided interfaces for monitoring, which may lead to incomplete views of the running status. For example, Lin \textit{et al.} \cite{lin2018tracking} noted that AWS Lambda's monitoring granularity is relatively coarse, and the tracking paths are not continuous across BaaS services.
% solutions (e.g., AWS X-Ray) cannot trace the invocation paths across BaaS services \cite{lin2018tracking}.
% \paragraph{C4: Monitoring and tracing are challenging in serverless.} % owing to the ephemerality of functions.}
% Apart from complicating security management tasks, serverless applications' broken boundaries also affect monitoring and tracing.
% Without the control of execution environment and BaaS services, monitoring relies on the interfaces exposed by providers. Thus developers may not have a complete view of the application's running status.
% Besides,  %Functions are instantiated and eliminated all the time, and
% The generated overwhelming logs also challenge the analysis system's insight capability.

%Due to performance and boot-time limitations, they may not be suitable for serverless scenarios.



% \paragraph{C3: Insecure third-party functions and packages may introduce vulnerabilities.}
%Like other programs, serverless applications can be affected by insecure third-party functions and packages.

% These runtimes are guaranteed to be up to date. %other software services are maintained by the provider and guaranteed to be up to date.

% Therefore, reliable monitoring are essential to defend against security risks contained in third-party software packages and functions.

% Consumers, instead of providers, are responsible for their maintenance and update.
% Besides, providers like AWS and Azure establish function marketplaces to facilitate developers. This could be risky in terms of security, and the challenges in security management (C2) and monitoring (C4) may further exacerbate this risk.
%https://aws.amazon.com/cn/serverless/serverlessrepo/
%https://azure.microsoft.com/en-us/marketplace/

\soa To address this challenge, researchers have attempted to mine and track the information flows in serverless applications from both static and dynamic perspectives.
Obetz \textit{et al.} \cite{obetz2019static} proposed an augmented call graph that considers BaaS services and explained the feasibility of obtaining the graph through static analysis.
To dynamically track where and how data flow, Datta \textit{et al.} \cite{datta2020valve} placed an agent in each function's container to proxy its network requests. These agents generated and propagated labels for inbound and outbound traffic to record the flow of information and could also restrict functions' behavior based on preconfigured policies. In addition, Lin \textit{et al.} \cite{lin2018tracking} proposed GammaRay, a dynamic tracking tool that can capture the causality of invocations across BaaS services to build complete trace graphs.

% \paragraph{R3: Information Flow Control.}
% Third-party functions is inevitable. To prevent the ensuing risks, existing works employ \textit{information flow control} to manage where and how the data are flowing \cite{datta2020valve,alpernas2018secure}.
% Generally, they put an agent in each function's container to proxy its network requests. These agents generate and propagate labels for inbound and outbound traffics to record data flows. Meanwhile, they conduct security enforcement according to pre-configured policies to restrict functions' behavior.



% \paragraph{R4: Invocation Relationship Mining.}
% Regarding monitoring and tracing, current research mainly focuses on obtaining the invocation relationship between functions, involving both static and dynamic methods.

% On the contrary, Lin \textit{et al.} \cite{lin2018tracking} proposed a dynamic tracking tool, GammaRay. It captures the causality of invocation events across BaaS services, thereby building a complete trace graph.

\ins Commercial platforms provide various tools and interfaces to record, aggregate, display, and analyze monitoring data. Some can even serve as triggers for automatic function management. They also aim to gradually enable distributed tracing while ensuring adequate performance.
Moreover, to further mitigate the impact of nonsecure third-party components, providers recommend continuous security validation in continuous integration and continuous deployment (CI/CD) pipelines and offer a series of tools, such as static vulnerability scanning and automatic penetration testing, for this purpose.


% \paragraph{P3: Security in the Development Phase.}
% To mitigate the impact of insecure third-party functions, providers recommend continuous security validation in the development phase (e.g., static vulnerability scanning, automatic penetration testing), and provide a set of tools for that.
% At runtime, multi-level security management (P2) and monitoring (P4) assume the responsibility of protecting serverless applications.

% \paragraph{P4: Monitoring and Tracing Tools.}



% Besides, Lin \textit{et al.} points out that current solutions (e.g., AWS X-Ray) cannot trace the invocation paths across BaaS services \cite{lin2018tracking}.

\rev
The proposed dynamic methods solve the problem of the coarse-grained and incomplete nature of the existing monitoring schemes to a certain extent. For example, data-oriented tracing \cite{datta2020valve} can be integrated with traditional behavior-oriented mechanisms.
Moreover, since functions have relatively low internal complexity, static-analysis-based methods are feasible. These approaches could be an effective supplement to dynamic methods, which may introduce considerable runtime overhead.
Following best practices in the development phase can also mitigate the threat posed by nonsecure third-party components.
Unfortunately, the information that can be obtained through static analysis is limited. Current dynamic solutions all require code instrumentation or agent embedding to enable end-to-end monitoring and tracking, resulting in high compilation and runtime overheads \cite{datta2020valve,lin2018tracking}.
Hence, we consider this challenge only partially resolved.


\reo
The exploration of nonintrusive tracking schemes is a potential research opportunity.
Furthermore, advanced insight capabilities are lacking in current platforms.
These capabilities include assessing security status, predicting and diagnosing faults, and conducting detection and forensics for security events. With various triggers, serverless applications can naturally perform ``feedback regulation'' for self-management.
Meanwhile, functions' short lifecycles and massive logs impose high requirements on the speed of solutions. We believe this scenario represents a research opportunity where artificial intelligence (AI)-based methods might be beneficial.





% \test{This
% % Currently, besides the integration with BaaS services, the main problems with this approach are performance issues and agents' intrusiveness.

% Continuous verification in development and fine-grained management at runtime largely mitigate threats of insecure third-party functions and libraries.}
% \paragraph{O3: More Runtime Defense Solutions for Third-Party Functions and Packages.}
%  Nonetheless, since customers are responsible for maintaining custom runtimes, it is essential to observe and restrict third-party components' behavior at runtime. In this respect, current research works are mainly information flow control based on taint propagation. Serverless will embrace more runtime defense solutions.

% \paragraph{O4: Fine-Grained and Non-Intrusive Monitoring and Tracing.}
% \test{

% However, current implementations are only transplantations of technologies used in microservices. Monitoring stays at the function level, which is coarse-grained and lacks instance-related insights. The instrumentation-based distributed tracing is also not suitable for serverless due to its inherent performance issues. }

% Relying on interfaces exposed by providers, serverless monitoring is coarse-grained and inflexible. Traditional distributed tracing systems are also intrusive and may encounter performance issues. Besides, BaaS services are embedded and work as components of the application, resulting in incomplete tracing.
% Therefore, for serverless applications, we need richer and more flexible monitoring options, as well as non-intrusive end-to-end tracing that can cover BaaS services.



==> Serverless Security [IEEE Network] (preprint)/texts/challenge_3_management.tex <==
\section{Challenge 3: Security Management}
\label{sec:management}

% \paragraph{C2: Security management becomes difficult due to the flexibility and complexity of serverless.}
% Functions work based on the event-driven model. The events that can cause function execution are called \textit{triggers}.
% Apart from HTTP invocations, providers offer various triggers such as queues, logs, storage, and timers. Benefiting from this, developers can easily integrate BaaS services to build flexible and scalable applications.

Security management is a critical means for administrators to enforce security intentions and protect applications. As described in \autoref{sec:threat}, the diversity of the possible attacks in serverless environments necessitates comprehensive security management capabilities that can provide protection at multiple levels.

However, the fragmented application boundaries of serverless applications increase the difficulty of security management. The distributed nature of functions further exacerbates this challenge.
On the one hand, functions must carefully inspect the input and output at all their entry points; failure to comply with this principle may lead to injection attacks. On the other hand, an external request may trigger communication among multiple functions and BaaS services, necessitating fine-grained authentication and authorization among functions and services. This task can be challenging for large-scale or complex applications.

% Moreover, diverse attack methods towards serverless applications require more comprehensive security management capabilities that can provide protection at multiple levels. For example, employing functions' stateless nature, adversaries may send numerous fraudulent requests to launch resource exhaustion attacks.
% Adversaries in the network may also perceive sensitive information from the communication pattern and active level of functions. Case in point: in a health monitoring application, a particular sequence of triggered functions may reflect a certain health condition of the patient \cite{shafiei2020serverless}.


% \paragraph{R2: Secure Container Network.}

\soa
% Since functions work together to provide services, it is necessary to perform fine-grained control over inter-function communication. % to guarantee the entire application's security.
Traditional authentication and authorization mechanisms have been well studied. Building on this work, researchers are currently attempting to provide advanced security management capabilities at new levels.
Sankaran \textit{et al.} \cite{sankaran2020workflow} built a workflow-sensitive authorization mechanism for serverless applications. It proactively verifies external requests' permissions for all functions involved in their workflows at the application entry point. Thus, applications can reject illegal requests as early as possible, thereby avoiding partial processing of illegal requests and reducing the potential attack surface.
Moreover, Nam \textit{et al.} \cite{nam2020bastion} revealed a data leakage risk in container networks and redesigned a secure network stack to protect intercontainer communication.
Specifically, the method verifies and filters out illegal requests based on the intercontainer dependencies and utilizes end-to-end direct forwarding to prevent traffic exposure. It even improves the container network's performance.



%However, the dependency maps are obtained from security management policies, so it still requires administrators' careful and correct configuration.


\ins Based on various security policies, cloud providers have formulated ``best practices'' for security management.
These policies act on multiple layers and multiple resources and have the potential to provide promising management capabilities.
For example, commercial platforms achieve well-defined identity authentication and fine-grained authorization with mature identity access management (IAM) systems.
AWS Lambda even provides role-based policies, resource-based policies, access control lists, and other management methods for consumers to choose among and flexibly combine.


% Operation security mechanisms are mainly about identity management and access control, which are utilized for authentication and authorization during function operations (e.g., creation, modification) and invocations.

\rev
Based on fine-grained security management policies, existing solutions provide multilevel protection for serverless applications. Providers also document best practices as guidance.
However, a gap may inevitably exist between actual situations and the recommended best practices.
First, both academic \cite{sankaran2020workflow,nam2020bastion} and industrial solutions require administrators to customize security policies in accordance with the application architecture and business logic. Although server management is the providers' responsibility, the burden placed on consumers for security management has not been relieved but instead has been made even heavier: fine-grained policies require attentive design and careful configuration, which is a time-consuming and error-prone process.
Second, providers' marketing emphasizes only cost-effectiveness and convenience, making it easy for consumers to ignore their responsibility to ensure security. As mentioned above, any violation of design principles and best practices may compromise applications' security.
In other words, current mechanisms do not reduce the complexity of security management. Applications' safety depends on the extent to which best practices are followed.
Therefore, we consider this challenge partially resolved.

\reo
At present, the assistance of automated tools is urgently needed. One possible research direction is automated security configuration. The ideal tool would be able to perceive an application's architecture and status, extract the consumer's security intentions, and provide support for policy configuration, maintenance, and updating.
%Some attempts are being made in this regard \cite{li2019towards}.
Another research direction concerns automated security audits, for which there is a growing market. The ideal tool is expected to not only check whether security measures are deployed but also evaluate the quality of these measures based on an application's specific characteristics.
We believe that the security risks posed by incorrect configurations can be alleviated by advancing research in these two directions.


==> Serverless Security [IEEE Network] (preprint)/texts/challenge_4_data.tex <==
\section{Challenge 4: Data Protection}
\label{sec:confidentiality}
Data security is the lifeline of cloud services. Unlike in other models, serverless providers control the whole application lifecycle (e.g., the deployment, scaling, execution, and termination of functions) and the entire software stack.
Moreover, as part of the application and business logic, BaaS services can directly access and process data. All these characteristics require consumers to have deep trust in the provider.

Nevertheless, whether during the execution of code in an uncontrolled environment or the processing of sensitive data through the platform's services, privacy and compliance concerns may arise. To alleviate these concerns, platforms need to implement strict data protection measures to clearly and fully persuade consumers.
Given the flexibility requirements of serverless environments, this task could be challenging, but it is essential for expanding the application scenarios of serverless computing.

% In the serverless model, the provider is responsible for managing the deployment, scaling, and execution of functions. The entire software stacks are also under its control.
% Therefore, protecting user data's confidentiality and integrity is a challenge for the expansion of serverless's application scenarios.

% \paragraph{C5: Privacy risks raised by running code in incompletely controlled environments.}
% How much should we trust the provider when deploying applications on cloud?
% For consumers, unreserved trust may be the last choice. %Unlike the platform as a service model,
% In serverless platforms, the entire software stacks are controlled by providers.
% to expand application scenarios, it is worth studying how to protect the confidentiality and integrity of data and code, mitigating consumers' disadvantaged position in terms of data security.



% \paragraph{R5: Hardware-Based Trusted Execution Environment.}
\soa
In addition to protecting data at rest or in transit through encryption, recent work has focused on protecting data in use.
Researchers have attempted to establish a \textit{trusted execution environment} (TEE) for functions to relieve customers of the need to fully trust providers \cite{qiang2018se, brenner2019trust}.
Specifically, several approaches employ Intel SGX, a hardware-based mechanism that uses encrypted memory to protect running code and data from privileged software, even the OS.
Moreover, Qiang \textit{et al.} \cite{qiang2018se} proposed a two-way sandbox, that is, a WebAssembly sandbox nested in an SGX sandbox, to prevent a platform from accessing sensitive data processed by functions while also protecting the platform from untrusted code.




\ins
% \paragraph{P5: Encryption in Transit and at Rest.}
% Data security is the lifeline of cloud services.
On the basis of their mature storage services and security management experience, commercial platforms provide adequate support for encryption in transit and at rest. This protection covers the files and code uploaded by customers as well as the environment variables of functions. Moreover, standard key management services (KMS) are provided to help customers handle secrets.


\rev
Protecting data in use has become a significant dimension of cloud security.
In this regard, current serverless research is focused on hardware-based TEEs, which still have many limitations, such as poor performance, difficulty with hardware heterogeneity, and running only in the user space.
Moreover, these techniques have not yet been applied to serverless products. Therefore, we consider this challenge to be partially resolved.

\reo
In recent years, many confidential computing solutions, such as homomorphic encryption and secure multiparty computation, have emerged for the protection of data in the cloud.
Considering the limitations of the current solutions, the community is expected to appreciate further exploration and adoption of these techniques.
% Taking into account the limitations of current solutions, the community will appreciate more exploration and adoption of these technologies.
% In terms of data protection, other confidential computing solutions  are emerging, such as homomorphic encryption and secure multi-party computation.






==> texts/4_solutions.tex <==


\oldparagraph{Countermeasures for the security concerns.} The responses to the concerns are mainly reflected in commercial platforms. 








%\paragraph{Findings and implications.}




%\xing{classify the mechanisms and map them to the research works and security concerns}

%\xue{You can adjust the format of this table later, I just want to see the effect.}




% \begin{table}[tb]
% \begin{tabular}{lllllll}
% \multicolumn{1}{c}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{Aspects}} & \multicolumn{1}{c}{\textbf{AWS Lambda}} & \multicolumn{1}{c}{\textbf{Google Cloud Functions}} & \multicolumn{1}{c}{\textbf{Azure Functions}} & \multicolumn{1}{c}{\textbf{Alibaba Function Compute}} & \multicolumn{1}{c}{\textbf{IBM Cloud Functions}} \\

% \multirow{3}{*}{Data Security} & Encryption in transit & function to filesystem, platform managent apis & support TLS & .... & support TLS & support \\
%  & Static encryption & files, secrets, environment variables & support & ... & .. & support \\
%  & isolation & Firecracker/container/microVM & ... & ... & ... & docker container \\
% \multirow{2}{*}{Operation Security} & authentication & .. & ... & ... & .. & .. \\
%  & Authorization & ... & ... & ... & .. & .. \\
% \multirow{2}{*}{Infrastructure Security} & Hardware & .. & ... & ... & .. & .. \\
%  & Software & .. & ... & ... & .. & .. \\
% \multirow{3}{*}{Monitoring} & Visualization & Amazon CloudWatch & Stackdriver Logging & Azure Monitor/application insights & CloudMonitor & sisdig \\
%  & Metrics? & .. & .. & .. & .. & .. \\
%  & Log & .. & .. & .. & .. & .. \\
% Tool & Tool &  &  & .. &  & 
% \end{tabular}
% \end{table}

==> texts/5_future.tex <==






